Verification of Geometric Robustness of Neural Networks via Piecewise Linear Approximation and Lipschitz Optimisation

We address the problem of verifying neural networks against geometric transformations of the input image, including rotation, scaling, shearing, and translation. The proposed method computes provably sound piecewise linear constraints for the pixel values by using sampling and linear approximations in combination with branch-and-bound Lipschitz optimisation. The method obtains provably tighter over-approximations of the perturbation region than the present state-of-the-art. We report results from experiments on a comprehensive set of verification benchmarks on MNIST and CIFAR10. We show that our proposed implementation resolves up to 32% more verification cases than present approaches.

==> sections/abstract.tex <==
%%%
    We address the problem of verifying neural networks against
    geometric transformations of the input image, including rotation,
    scaling, shearing, and translation. The proposed method computes
    provably sound piecewise linear constraints for the pixel values
    by using sampling and linear approximations in combination with
    branch-and-bound Lipschitz optimisation.  A feature of the method
    is that it obtains tighter bounds than present state-of-the-art.
    We report results from experiments on a set of benchmark networks
    from VNN20 showing that our proposed implementation was able to
    resolve more verification cases than the present approaches while being more computationally efficient.
%AL: At lower cost?

    %AL: would be


%We report the experiments obtained
%
%AL: NEeds to be quantified for the abstract in the paper (no need for
%the abstract submission).
     %% demonstrate the superior performance of the method proposed here
    %% compared to the SoA approaches in terms of both verification
    %% accuracy and computational time.



%AL: Updated.
%%     Robustness verification of neural networks against a specified
%%     threat model is important in safety-critical applications. Most
%%     existing verification methods focus on the norm-based threat model
%%     of pixel perturbations, but they cannot address semantic attacks
%%     defined by natural geometric transformations, \textit{e.g.}, rotation,
%%     scaling, and lighting perturbations. Unlike the norm-based pixel
%%     perturbations that define a convex input set, the input instances
%%     obtained through geometric transformations form a highly nonconvex
%%     set, posing a significant challenge for the verification problem.
%%     %
%%     % The SoA can at present address only relatively small networks,
%%     % against relatively small geometric perturbations.
%%     % The statement above is not very precise. ETH paper has experiments on large networks
%%     %
%%     %We address this challenge by introducing novel piecewise linear
%%     %relaxations for geometric transformations with respect to the
%%     %parameter space (e.g., the rotation angle). A sequence of sampling,
%%     %linear optimisation, and branch-and-bound Lipschitz procedure are
%%     %used to compute sound piecewise linear constraints. Our piecewise
%%     %linear relaxation method is provably tighter than the
%%     %state-of-the-art (SoA) approaches based on interval bounds and
%%     %linear relaxations. Experiments on a set of benchmark networks
%% %AL: specify the experiment
%%     %demonstrate the superior performance of the method proposed here
%%     %compared to the SoA approaches in terms of both verification
%%     %accuracy and computational time.
%%     %%%%%%%%
%% %AL: my suggested ver:
%% %
%%     We address the challenge of verifying neural networks against
%%     geometric transformations. The proposed method computes provably
%%     sound piecewise linear constraints for the pixel values by using
%%     sampling and linear approximations in combination with branch-and-bound
%%     Lipschitz optimisation.  By doing so we obtain provably tighter bounds
%%     than present state-of-the-art
%%     approaches. %We report the experiments obtained
%% %
%%     Experiments on a set of benchmark networks from VNN20 demonstrate
%%     that the present method achieves tighter accuracy and
%%     lower computational cost than the present state-of-the-art.
%% %AL: NEeds to be quantified for the abstract in the paper (no need for
%% %the abstract submission).
%%      %% demonstrate the superior performance of the method proposed here
%%     %% compared to the SoA approaches in terms of both verification
%%     %% accuracy and computational time.


==> sections/geo_transformation.tex <==

a list of geometric transformation

==> sections/proofs.tex <==

Here, we complete the proofs for Propositions~\ref{prop:linear_optimisation}-\ref{proposition:gradient}.

\subsection{Proof of Proposition~\ref{prop:linear_optimisation}}
Consider the piecewise linear function in the objective function~\eqref{eq:bound_sample_optimisation}. Let $\mathcal{B}_j, j = 1, \ldots, q$ be the effective piecewise domain of the $j$th segment, \textit{i.e.},
\begin{equation} \label{eq:piecewise_domain}
    \max_{j = 1,\ldots,q} \{\underline{w}_j^\tr \kappa_i + \underline{b}_j\} = \begin{cases}
    \underline{w}_1^\tr \kappa_i + \underline{b}_1, & \text{if} \quad \kappa_i \in \mathcal{B}_1 \\
    \underline{w}_2^\tr \kappa_i + \underline{b}_2, & \text{if} \quad \kappa_i \in \mathcal{B}_2 \\
    \quad \vdots \\
    \underline{w}_q^\tr \kappa_i + \underline{b}_q, & \text{if} \quad \kappa_i \in \mathcal{B}_q.
    \end{cases}
\end{equation}
Then, the objective function~\eqref{eq:bound_sample_optimisation} can be equivalently written into
\begin{equation*}
\begin{aligned}
&\frac{1}{N}\sum_{i=1}^N \left(\mathcal{G}_{u,v}(\kappa_i) - \big(\max_{j = 1,\ldots,q} \{\underline{w}_j^\tr \kappa_i + \underline{b}_j\}\big)\right) \\
= &\frac{1}{N}\sum_{j=1}^q\left(\sum_{\kappa_i \in \mathcal{B}_j }\left(\mathcal{G}_{u,v}(\kappa_i) - \big(\underline{w}_j^\tr \kappa_i + \underline{b}_j\big) \right)\right)
\end{aligned}
\end{equation*}
Therefore,~\eqref{eq:bound_sample_optimisation} is equivalent to
\begin{equation}\label{eq:bound_sample_optimisation_s2}
    \begin{aligned}
      \min_{\underline{w}_j, \underline{b}_j, \mathcal{B}_j, j = 1, \ldots, q} \quad & \sum_{j=1}^q\left(\frac{1}{N}\sum_{\kappa_i \in \mathcal{B}_j }\left(\mathcal{G}_{u,v}(\kappa_i) - \big(\underline{w}_j^\tr \kappa_i + \underline{b}_j\big) \right)\right) \\
        \text{subject to} \quad &  \underline{w}_j^\tr \kappa_i + \underline{b}_j \leq \mathcal{G}_{u,v}(\kappa_i), \\
        & \quad i = 1, \ldots, N, j = 1, \ldots q.
    \end{aligned}
\end{equation}
Note that the piecewise domains $\mathcal{B}_j$ are determined by the linear segments $\underline{w}_j, \underline{b}_j, j = 1, \ldots, q$ implicitly in~\eqref{eq:piecewise_domain}. We need to simultaneously optimize the choices of $\mathcal{B}_j$ in~\eqref{eq:bound_sample_optimisation_s2}, making it computationally hard to solve.

A suboptimal solution for~\eqref{eq:bound_sample_optimisation_s2} is to \emph{a priori} fix the effective domain $\mathcal{B}_j$ and optimize over $\underline{w}_j, \underline{b}_j, j = 1, \ldots, q$ only, i.e.,
\begin{equation}\label{eq:bound_sample_optimisation_s2}
    \begin{aligned}
       \hat{\beta} := \min_{\underline{w}_j, \underline{b}_j, j = 1, \ldots, q} \; & \sum_{j=1}^q\left(\frac{1}{N}\sum_{\kappa_i \in \mathcal{B}_j }\left(\mathcal{G}_{u,v}(\kappa_i) - \big(\underline{w}_j^\tr \kappa_i + \underline{b}_j\big) \right)\right) \\
        \text{subject to} \quad &  \underline{w}_j^\tr \kappa_i + \underline{b}_j \leq \mathcal{G}_{u,v}(\kappa_i), \\
        & \quad i = 1, \ldots, N, j = 1, \ldots q,
    \end{aligned}
\end{equation}
which is decoupled into $q$ individually linear programs, $j = 1, \ldots, q$
\begin{equation}\label{eq:bound_sample_optimisation_individual_s2}
    \begin{aligned}
      \beta^*_j :=  \min_{\underline{w}_j, \underline{b}_j} \quad & \frac{1}{N}\sum_{\kappa_i \in \mathcal{B}_j }\left(\mathcal{G}_{u,v}(\kappa_i) - \big(\underline{w}_j^\tr \kappa_i + \underline{b}_j\big) \right) \\
        \text{subject to} \quad &  \underline{w}_j^\tr \kappa_i + \underline{b}_j \leq \mathcal{G}_{u,v}(\kappa_i), \; i = 1, \ldots, N.
    \end{aligned}
\end{equation}
Therefore, it is clear that $\hat{\beta} = \sum_{j=1}^q \beta^*_j \geq \beta^*$.

On the other hand, suppose the optimal solution to~\eqref{eq:bound_sample_optimisation} leads to the optimal effective domains $\mathcal{B}_j,j = 1, \ldots, q$ in~\eqref{eq:piecewise_domain}. Then, using this set $\mathcal{B}_j,j = 1, \ldots, q$, the decoupled linear programs~\eqref{eq:bound_sample_optimisation_individual_s2} are equivalent to~\eqref{eq:bound_sample_optimisation_s2} and~\eqref{eq:bound_sample_optimisation}. This completes the proof.

%\vspace{5mm}

\subsection{Proof of Proposition~\ref{prop:lipschitz_constants}}
Recall the definition of the violation function
$$
\underline{f}_{u, v}(\kappa) := \max_{j =
   1,\ldots,q} \{\underline{w}_j^\tr \kappa_i + \underline{b}_j\} -
   \mathcal{G}_{u,v}(\kappa)
$$
in which the pixel value function is given by
$
    \mathcal{G}_{u,v}(\kappa) := \mathcal{P}_{\alpha, \beta} \circ \mathcal{I} \circ \mathcal{T}^{-1}_\mu(u,v).
$
We know that the spatial transformation $\mathcal{T}_{\mu}(u,v)$ and $\mathcal{P}_{\alpha, \beta}$ are continuous and differentiable everywhere. The interpolation function $\mathcal{I}(u,v)$ is continuous everywhere, but it is only differentiable within each interpolation region and it can be nonsmooth on the boundary. Also, $\mathcal{T}_{\mu}(u,v)$ and $\mathcal{I}(u,v)$ are generally nonconvex.

In addition, the piecewise linear function
$$\max_{j =
   1,\ldots,q} \{\underline{w}_j^\tr \kappa_i + \underline{b}_j\}$$
    is continuous but not differential everywhere. Therefore, the violation function $\underline{f}_{u, v}(\kappa)$ is nonconvex and nonsmooth in general. Finally, all the functions $\mathcal{T}_{\mu}(u,v)$, $\mathcal{P}_{\alpha, \beta}$, $\mathcal{I}(u,v)$ and $\max_{j =
   1,\ldots,q} \{\underline{w}_j^\tr \kappa_i + \underline{b}_j\}$ are Lipschitz continuous, so is the violation function $\underline{f}_{u, v}(\kappa)$. Thus, there exist
   $L_i > 0$, $i = 1, \ldots, d$, such that \eqref{eq:Lipschitz_bound} holds.

%\vspace{5mm}

\subsection{Proof of Proposition~\ref{proposition:gradient}}
This proof is motivated by~\cite{jordan2020exactly}. In order to prove Proposition~\ref{proposition:gradient}, we first state a useful result from~\cite[Lemma 3]{jordan2020exactly}.

Let $f(x):\mathbb{R}^n \rightarrow \mathbb{R}$ be Lipschitz continuous over an open set $\Omega \subset \mathbb{R}^n$. We denote $\mathrm{Diff}(\Omega)$ as the subset of $\Omega$ where $f(x)$ is differentiable. We also let $\mathcal{D}$ be the set of $(x,v) \in \mathbb{R}^{2n}$ for which the directional derivative
$$
    \nabla_v f(x) := \lim_{t \rightarrow 0} \frac{f(x + tv) - f(x)}{t}
$$
exists and $x \in \Omega$. Finally, we let $\mathcal{D}_v$ be the set
$
    \mathcal{D}_v = \{x \in \mathbb{R}^n\mid (x,v) \in \mathcal{D}\}.
$
Then, we have the following inequality~\cite[Lemma 3]{jordan2020exactly}
\begin{equation} \label{eq:derivative_inequality}
    \sup_{x \in \mathcal{D}_v} |\nabla_v f(x)| \leq \sup_{x \in \mathrm{Diff}(\Omega)} |\nabla f(x)^\tr v|.
\end{equation}

We now precede to prove Proposition~\ref{proposition:gradient}.
%
Fix any $\kappa_1, \kappa_2 \in \mathcal{B}$, and we define a function $h(t): \mathbb{R} \rightarrow \mathbb{R}$ as
$$
    h(t) = \underline{f}_{u, v}(\kappa_1 + t(\kappa_2-\kappa_1)).
$$
Since $\underline{f}_{u, v}(\kappa)$ is Lipschitz continuous in $\mathcal{B}$, it is clear that $h(t)$ is Lipschitz continuous on the interval $[0,1]$. Thus, by Rademacher's Theorem, $h(t)$ is differentiable everywhere except for a set of measure zero.

We can further define a Lebesgue integrable function $g(t)$ that equal to $h'(t)$ almost everywhere as follows
$$
    g(t) = \begin{cases} h'(t), & \text{if} \quad h'(t) \quad \text{exists} \\
    \sup_{s \in [0,1]} |h'(s)|, &\text{otherwise}
    \end{cases}.
$$
Note that if  $\underline{f}_{u, v}(\kappa)$ is differentiable at some point, we have
$$
    h'(t) = \nabla \underline{f}_{u, v}(\kappa_1 + t(\kappa_2 - \kappa_1))^\tr (\kappa_2 - \kappa_1).
$$
Then we have the following inequalities
$$
\begin{aligned}
    |\underline{f}_{u, v}(\kappa_1) - \underline{f}_{u, v}(\kappa_2)| &= |h(1) - h(0)| \\
    &= \left|\int_0^1 g(t) dt\right| \\
    & \leq \int_0^1 |g(t)| dt \\
    &\leq \int_0^1 \sup_{s \in [0,1]} |h'(s)| dt \\
    &{= \sup_{s \in [0,1]} |h'(s)|} \\
    &{\leq \sup_{\kappa \in \mathcal{D}_{\kappa_2-\kappa_1}} |\nabla_{\kappa_2-\kappa_1} \underline{f}_{u, v}(\kappa)|}.
\end{aligned}
$$
Furthermore, considering the inequality in~\eqref{eq:derivative_inequality}~\cite[Lemma 3]{jordan2020exactly}, we have
$$
    \begin{aligned}
        &\quad |\underline{f}_{u, v}(\kappa_1) - \underline{f}_{u, v}(\kappa_2)| \\
        &{\leq \sup_{\kappa \in \mathrm{Diff}(\mathcal{B})} |\nabla \underline{f}_{u, v}(\kappa)^\tr  (\kappa_2 - \kappa_1)|} \\
    &\leq \sum_{i=1}^d \sup_{\kappa \in \mathrm{Diff}(\mathcal{B})} |\nabla \underline{f}_{u, v}(\kappa)^\tr e_i|  |\kappa_2(i) - \kappa_1(i)|
    \end{aligned}
$$
where $e_i \in \mathbb{R}^d$ is a basis vector with only the $i$-th element being one and the rest being zero. Therefore, the Lipschitz constants in~\eqref{eq:Lipschitz_bound} can be chosen as
    $
       L_i = \sup_{\kappa \in \mathrm{Diff}(\mathcal{B})} |\nabla \underline{f}_{u, v}(\kappa)^\tr e_i|.
    $
    This finishes the proof.
%The proof of the step highlighted in {\color{blue}blue} above requires \cite[Lemma 3]{jordan2020exactly}.



